Towards Vision Mixture of Experts for Wildlife Monitoring on the Edge

The explosion of IoT sensors in industrial, consumer and remote sensing use cases has come with unprecedented demand for computing infrastructure to transmit and to analyze petabytes of data. Concurrently, the world is slowly shifting its focus towards more sustainable computing. For these reasons, there has been a recent effort to reduce the footprint of related computing infrastructure, especially by deep learning algorithms, for advanced insight generation. The `TinyML' community is actively proposing methods to save communication bandwidth and excessive cloud storage costs while reducing algorithm inference latency and promoting data privacy. Such proposed approaches should ideally process multiple types of data, including time series, audio, satellite images, and video, near the network edge as multiple data streams has been shown to improve the discriminative ability of learning algorithms, especially for generating fine grained results. Incidentally, there has been recent work on data driven conditional computation of subnetworks that has shown real progress in using a single model to share parameters among very different types of inputs such as images and text, reducing the computation requirement of multi-tower multimodal networks. Inspired by such line of work, we explore similar per patch conditional computation for the first time for mobile vision transformers (vision only case), that will eventually be used for single-tower multimodal edge models. We evaluate the model on Cornell Sap Sucker Woods 60, a fine grained bird species discrimination dataset. Our initial experiments uses $4X$ fewer parameters compared to MobileViTV2-1.0 with a $1$% accuracy drop on the iNaturalist '21 birds test data provided as part of the SSW60 dataset.

==> sections/instructions.tex <==
\section{Submission of papers to NeurIPS 2024}


Please read the instructions below carefully and follow them faithfully.


\subsection{Style}


Papers to be submitted to NeurIPS 2024 must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long,
including figures. Additional pages \emph{containing only acknowledgments and
references} are allowed. Papers that exceed the page limit will not be
reviewed, or in any other way considered for presentation at the conference.


The margins in 2024 are the same as those in previous years.


Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.


\subsection{Retrieval of style files}


The style files for NeurIPS and other conference information are available on
the website at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2024.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.


The only supported style file for NeurIPS 2024 is \verb+neurips_2024.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}


The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.


\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit, as long as you do not say which conference it was submitted to. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS.


At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.


The file \verb+neurips_2024.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.


The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.


\section{General formatting instructions}
\label{gen_inst}


The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.


The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.


For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.


Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.


\section{Headings: first level}
\label{headings}


All headings should be lower case (except for first word and proper nouns),
flush left, and bold.


First-level headings should be in 12-point type.


\subsection{Headings: second level}


Second-level headings should be in 10-point type.


\subsubsection{Headings: third level}


Third-level headings should be in 10-point type.


\paragraph{Paragraphs}


There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.


\section{Citations, figures, tables, references}
\label{others}


These instructions apply to everyone.


\subsection{Citations within the text}


The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.


The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}


If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2024+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}


If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2024}
\end{verbatim}


As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous'' and include a copy of the anonymized paper in the supplementary material.


\subsection{Footnotes}


Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).


Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}


\subsection{Figures}


\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}


All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.


You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.


\subsection{Tables}


All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.


Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.


Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.


\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Math}
Note that display math in bare TeX commands will not create correct line numbers for submission. Please use LaTeX (or AMSTeX) commands for unnumbered display math. (You really shouldn't be using \$\$ anyway; see \url{https://tex.stackexchange.com/questions/503/why-is-preferable-to} and \url{https://tex.stackexchange.com/questions/40492/what-are-the-differences-between-align-equation-and-displaymath} for more information.)

\subsection{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.


\section{Preparing PDF files}


Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''


Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.


\begin{itemize}


\item You should directly generate PDF files using \verb+pdflatex+.


\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.


\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.


\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.


\end{itemize}


If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.


\subsection{Margins in \LaTeX{}}


Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})


A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.

\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2024/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to automatically hide this section in the anonymized submission.
\end{ack}

\section*{References}

References follow the acknowledgments in the camera-ready paper. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
Note that the Reference section does not count towards the page limit.
\medskip


{
\small


[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.


[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.


[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.
}

==> sections/rebuttal_page.tex <==
\setcounter{figure}{0} 
\setcounter{page}{1}
\begin{figure*}[ht!]
    \begin{center}
        \begin{tabular}{lllll}
            \includegraphics[width=.22\linewidth]{Styles/figures/placeholder_imagenet/birds_cluster.PNG} & \includegraphics[width=.22\linewidth]{Styles/figures/placeholder_imagenet/cat_cluster.PNG} & \includegraphics[width=.22\linewidth]{Styles/figures/placeholder_imagenet/dog_cluster.PNG} & \includegraphics[width=.22\linewidth]{Styles/figures/placeholder_imagenet/reptile_cluster.PNG} \\
             \includegraphics[width=.22\linewidth]{Styles/figures/placeholder_imagenet/human_cluster.PNG} & \includegraphics[width=.22\linewidth]{Styles/figures/placeholder_imagenet/fruits_cluster.PNG} &
            \includegraphics[width=.22\linewidth]{Styles/figures/placeholder_imagenet/text_cluster.PNG} & \includegraphics[width=.22\linewidth]{Styles/figures/placeholder_imagenet/building_cluster.PNG} \\
            % & \includegraphics[width=.28\linewidth]{Styles/figures/placeholder_imagenet/vehicle_cluster.PNG}\\
            \end{tabular}
    \caption{Sample patches assigned to different MoE-64 experts in the last MoE layer at initialization for ImageNet-1k using the Agglomerate clustering algorithm. The patches that are routed to different experts generally include species, text and structures that are either semantically similar or have similar visual features. Since ImageNet features a lot lot of fine-grained species, e.g. about 120 dog breeds, training on a subset of imagenet dataset would demonstrate generalizability of the model to other wildlife scenarios.}
    \label{fig:imagenet_semantic_splits}
    \end{center}
\end{figure*}

\begin{figure*}[ht!]
\begin{center}
    \begin{tabular}{c}
        \includegraphics[width=.95\linewidth]{Styles/figures/old_imnet_agg.pdf} \\
        
        $(a)$ \\
        \includegraphics[width=.95\linewidth]{Styles/figures/imnet_128_kmeans.pdf} \\
         $(b)$
        
    \end{tabular}
    \caption{Sample initialization expert affinity for the ImageNet-1k dataset, using 100 randomly sampled images per class from the training dataset. The plots are generated with embeddings from the last transformer block in the MobileViT model. The y-axis has been stretched by a factor of 4 (for a total of 64 experts) for visibility. $(a)$ is an expert affinity map generated using the Agglomerative clustering algorithm as in the rest of the paper with the top 128 representative patches from each of the 1000 classes. $(b)$ shows the same top $128$ patches used in $(a)$ but clustered with K-Means algorithm. Agglomerate clustering generates a more confident semantic split for imagenet and can be confirmed qualitatively as well.}
    \label{fig:affinity_2468}
\end{center}
\end{figure*}

% \begin{figure*}[ht!]
% \begin{center}
%     \begin{tabular}{cccc}
%         \includegraphics[width=.22\linewidth]{Styles/figures/experts_classes/64_fraction_cluster_layer_2.png} &

%         \includegraphics[width=.22\linewidth]{Styles/figures/experts_classes/64_fraction_cluster_layer_4.png} &
        
%         \includegraphics[width=.22\linewidth]{Styles/figures/experts_classes/64_fraction_cluster_layer_6.png} & 
        
%         \includegraphics[width=.22\linewidth]{Styles/figures/experts_classes/64_fraction_cluster_layer_8.png}  \\
        
%         % $(a)$ & $(b)$ & $(c)$ & $(d)$ \\
%     \end{tabular}
%     \caption{\scriptsize PLACEHOLDER: Cluster-class affinity using softmax temperature of $0.001$ and cut-off threshold of $0.05$ for layers $2,4,6,8$ in order for MoE-64 after 10\% imagenet finetuning.}
%     \label{fig:affinity_2468}
% \end{center}
% \end{figure*}

% \begin{figure*}[ht!]
% \begin{center}
%     \begin{tabular}{cccc}
%         \includegraphics[width=.22\linewidth]{Styles/figures/experts_classes/64_fraction_cluster_layer_2.png} &

%         \includegraphics[width=.22\linewidth]{Styles/figures/experts_classes/64_fraction_cluster_layer_4.png} &
        
%         \includegraphics[width=.22\linewidth]{Styles/figures/experts_classes/64_fraction_cluster_layer_6.png} & 
        
%         \includegraphics[width=.22\linewidth]{Styles/figures/experts_classes/64_fraction_cluster_layer_8.png}  \\
        
%         % $(a)$ & $(b)$ & $(c)$ & $(d)$ \\
%     \end{tabular}
%     \caption{\scriptsize PLACEHOLDER: From left to right is the finetuning router stability for random initialization, followed by KMeans, GMM Diagonal, GMM Spherical, Agglomerative. GMM router only uses the means. Including the covariance matrix would increase the router cost by a factor of $D$, where $D$ is the model dimension.}
%     \label{fig:affinity_clustering_algo}
% \end{center}
% \end{figure*}


% \begin{table}[!htbp]
%     \centering
%     \small
%     \caption{\scriptsize Ablation for MoE layers using MobileVitV2-0.5 as the backbone for 16 experts at $10$ epochs. (moelr, mlp latent dim, nexperts)}
%     \begin{tabular}{ccccc} \\ 
%     \hline
%       Layers & Parameters (millions) & Data Subset & Batch Size & Imagenet-1k \\
%     \hline
%      2,4,6,8 & TODO & 0.1 & 512 & TODO \\
%       & & 0.1 & 512 & TODO \\
%      \hline
%      2,4,6,8 & TODO & 0.1 & 512 & TODO \\
%      & & 0.5 & & TODO \\
     
%     \hline 
%     \end{tabular}
%     \label{tab:imagenet_vision_ablation}
% \end{table}

==> tables/ssw60_av.tex <==
\begin{table*}[!htbp]
    \centering
    \small
    \begin{tabular}{cccccc} \\ \hline
     Visual PT    & Audio PT  & MBT (score) & MobileNet (fusion)  & MobileViT (fusion)  & MobileViTMoE (single tower) \\ \hline 
     Imagenet    & Imagenet   & 58.9        & {\color{red}{50.77}} & {\color{red}{50.20}} & {\color{red}{TODO}} \\
     % Imagenet    & iNat Audio & 63.5        & {\color{red}{TODO}} & {\color{red}{TODO}} & {\color{red}{TODO}} \\
     iNat Images & iNat Audio & 80.6        & {\color{red}{TODO}} & {\color{red}{TODO}} & {\color{red}{TODO}} \\
     % Audioset    & Audioset   & -           & {\color{red}{TODO}} & {\color{red}{TODO}} & {\color{red}{TODO}} \\
    \hline
    \end{tabular}
    \caption{\textit{Pretraining effect on SSW60 Audio-Visual classification. Comparison of mobile models audio-visual SSW60 video classification with the baseline (MBT). Similar to the baseline, we combine the validation setup of audio and video frames in audio-visual experiments. PT Refers to the pretrain data for each modality. \textcolor{red}{THIS WILL BE UPDATED TO RESULTS FOR BIRDS INAT AUDIO VISUAL}}}
    \label{tab:ssw60_av}
\end{table*}

==> tables/ssw60_direct_eval.tex <==

Next, we test the performance of the mixture of experts model on the fine grained SSW60 video dataset. 

\begin{table}[!htbp]
    \centering
    \small
    \begin{tabular}{cccc} \\ 
    \hline
     FT & Model & iNat'21 Birds Images & SSW60 Video \\
    \hline
     & ResNet50 & 60.47 & 54.92 \\
    Yes & ResNet50 & 71.88 & - \\
     & EfficientNet-B4 & 46.03 & 55.73 \\
    Yes & EfficientNet-B4 & 72.14 & - \\
     & MobileNetV2 & 12.07 & 40.14 \\
    Yes & MobileNetV2 & 47.57 & - \\
     & MobileViT & 10.84 & 39.37 \\
    Yes & MobileViT & 50.05 & - \\
     % & MobileViTMoE-2 & \textcolor{orange}{10.11} & \textcolor{orange}{TODO} \\
    % Yes & MobileViTMoE-2 & \textcolor{orange}{TODO} & - \\
    % & MobileViTMoE-8 & TODO & TODO \\
    % Yes & MobileViTMoE-8 & TODO & - \\
    & MobileViTMoE-16 & orange{10.01} & 28.63 \\
    Yes & MobileViTMoE-16 & 46.02 & - \\
     & MobileViTMoE-64 & 10.16 & 32.6 \\
    Yes & MobileViTMoE-64 & 52.1 & - \\
    \hline
    \end{tabular}
    
    \caption{\textit{SSW60 Vision Evaluation experiments. For each model, the first row shows training on birds inat or SSW60 and evaluating directly on SSW60. The second row finetunes the model trained on birds inat with SSW60 before evaluation.}}
    
    % \textcolor{red}{The SSW60 vision training looks off at the moment - likely due to data loader issue. I'm pausing discussion on this table until that is sorted. If not fixed before deadline, we will stick to the birds inat result from Table \ref{tab:birds_inat_vision_eval}; Updates: It looks like this might be because ssw60 needs it own router cluster init. on that atm; Updates: the code to generate the clusters is fixed for the video data and will move forward to that set of experiments in case we can still include}}
    \label{tab:ssw60_vision_eval}
\end{table}
